Cross-Layer TopK: Dynamically Allocating Sparsity Across Layers in Transcoders

Cross-Layer Transcoders (CLTs) decompose the activations of large language models into human-interpretable features and trace how these features interact across layers to form circuits, making them a key tool for mechanistic interpretability. However, training CLTs effectively and efficiently is hard. Beyond the usual trade-off between sparsity and reconstruction quality, a CLT has to model all layers at once, which adds a further challenge. The common JumpReLU recipe controls sparsity only indirectly through a penalty, while the direct extension of TopK selects a fixed number of latents in every layer. Yet reconstruction difficulty differs widely across layers, and intermediate layers are much harder than others, so giving every layer the same budget is suboptimal. We propose Cross-Layer TopK, which sets a single L0 budget for the whole model and dynamically allocates it across layers during training. In a comparison with JumpReLU and other TopK variants on Qwen3-8B-Base, this gives lower FVU while using 20% fewer active latents than JumpReLU. The better reconstruction carries over to circuit tracing, yielding more complete circuits with higher replacement and completeness scores. The fixed per-token budget of Cross-Layer TopK also makes it easy to pair with sparse decoding, which cuts both computation and communication and gives a 2.9x speedup per training step. We further show that Cross-Layer TopK follows scaling laws in both latent size and sparsity. We have open-sourced the weights of our CLT at https://huggingface.co/ByteDance-Seed/Cross-Layer-TopK-CLT.

==> sections/Results/Metrics.tex <==
\subsubsection{Metrics}

We primarily use the Fraction of Variance Unexplained (\textbf{FVU}) to evaluate the reconstruction performance of our CLTs.

We define the FVU of layer $l$ as
\[
\fvu{l} = \frac{\mathbb{E}\left[\left\lVert \mlpout{l}  -  \recon{l}\right\rVert_2^2\right]}{\mathbb{E}\left[\left\lVert \mlpout{l} - \bar{\mlpout{}}^{l}\right\rVert_2^2\right]},
\]

where $\bar{\mlpout{}}^{l} = \mathbb{E}[y^l]$, and the expectations are taken over the data distribution (activation groups with lengths over 20 times the mean are filtered). Then the \textbf{overall FVU} is defined by the average of FVU across all layers, i.e.

\[
\FVU = \frac{1}{L}\sum_{l=1}^{L} \fvu{l},
\]
which serves as our primary single-number summary of a CLT's reconstruction fidelity.


==> sections/Results/Training_Data.tex <==
\subsection{Training Data}

We trained our CLT on Qwen3-8B-Base~\citep{yang2025qwen3} activations using a mixture of pre-training and post-training data of Olmo 3~\citep{olmo2025olmo3} training dataset. $5/8$ of activations are generated from a pre-training dataset, $1/4$ of activations are generated from a reasoning Chain-of-Thought dataset, and $1/8$ are generated from an instruction following SFT dataset.

We maintained a pool of activations of size $163840 = 10 \times 2^{14}$, where one \emph{group} of activations refers to the MLP inputs and outputs at all layers produced by a single token; each slot in the pool thus holds one such group. For each example in the dataset, we ran a forward pass of the LLM to obtain, for every token, the input to and output of the MLP submodule at each layer, and then sampled only $512$ groups of activations (i.e., the activations of $512$ tokens) from that example into the pool, discarding the remaining activations. We trained CLT with gradient accumulation. For each micro-batch, we uniformly at random drew a micro-batch-size number of groups of activations from the pool for training and removed them from the pool. The LLM then continued to load data and run forward passes to refill the pool, and only once the pool was full did we proceed to the next micro-batch. This procedure helps increase the diversity of the activation sources within a single (large) batch. \Cref{app:training_setting} gives the optimization and initialization settings, including the micro-batch size and the number of accumulation steps.


==> sections/Sparse_Decode.tex <==
\section{Sparse Decode}
\label{sec:sparse_decode}

Because \textbf{CLTK} fixes the number of active latents per token in advance, the decoder never
has to be evaluated at the latents that were not selected. We exploit this in the training
infrastructure. We follow existing transcoder design notes~\citep{lindsey2025landscape} and
implement a sparse decoding scheme for CLT training. As is shown in \Cref{fig:sparse_decode}, we
(i) keep the encoder sharded along the feature axis $F$, (ii) shard the decoder along the model
dimension $D$, and (iii) exchange only Top-K activations across ranks. This removes the dense
reconstruction all-reduce that dominates communication in other sharding methods. Finally, the
per-token loss tensor is all-reduced. \Cref{alg:sparse_decode} shows the pseudocode of sparse
decoding.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.95\linewidth]{resources/sparse_decode.pdf}
    \caption{The sparse decoding scheme. The encoder stays sharded along the feature axis $F$, the
    decoder is sharded along the model dimension $D$, and only the Top-K activations are
    exchanged across ranks, which avoids the dense reconstruction all-reduce.}
    \label{fig:sparse_decode}
\end{figure}

Following the convention of the literature that discusses transcoder implementations, this section
refers to the two sharded axes as the feature axis $F$ and the model dimension $D$, which are the
latent size $m$ and the model dimension $n$ of \Cref{CLT}. Throughout this section, $B$ is the number
of tokens in a micro-batch, $W$ the number of ranks, $L$ the number of layers and $K$ the number of
active latents per token, with $F_{\mathrm{loc}} = F / W$ and $D_{\mathrm{loc}} = D / W$ denoting
the shard held by one rank. Layers are indexed from $0$ to $L-1$, and $\mathrm{nnz}_i$ is the
number of active latents that layer $i$ contributes to a micro-batch.

\begin{algorithm}[t]
\caption{Sparse decode for one CLT training step on $W$ ranks}
\label{alg:sparse_decode}
\begin{algorithmic}[1]
\Require MLP inputs $X$, encoder shard $W_{\mathrm{enc}}$ of shape $(L, F_{\mathrm{loc}}, D)$,
decoder shards $W_{\mathrm{dec}}$ with $W_{\mathrm{dec}}[i]$ of shape $(F, L-i, D_{\mathrm{loc}})$,
kernel \texttt{mode}, one of \texttt{dense}, \texttt{gather} or \texttt{embedding\_bag}
\Statex
\Procedure{TrainStep}{$X$}
    \State $\mathrm{acts} \gets$ \textproc{TopK}(\textproc{Einsum}(\texttt{bld,lfd->blf}, $X$, $W_{\mathrm{enc}}$))
        \Comment{$(B, L, F_{\mathrm{loc}})$}
    \State $\mathrm{sparse} \gets$ \textproc{AllReduceSum}(\textproc{Coo}($\mathrm{acts}$, \texttt{feat\_offset} $= \mathrm{rank} \cdot F_{\mathrm{loc}}$))
        \Comment{four tensors of length $\mathrm{nnz}$}
    \State \Return \textproc{SparseDecode}($\mathrm{sparse}$, $W_{\mathrm{dec}}$, \texttt{mode})
        \Comment{$(B, L, D_{\mathrm{loc}})$}
\EndProcedure
\Statex
\Procedure{SparseDecode}{$\mathrm{sparse}$, $W_{\mathrm{dec}}$, \texttt{mode}}
    \State $\mathrm{vals}, \mathrm{rows}, \mathrm{cols}, \mathrm{slices} \gets$ \textproc{SortByLayer}($\mathrm{sparse}$)
        \Comment{$\mathrm{slices}[i]$ is the range of layer $i$}
    \State $\mathrm{recon} \gets \mathbf{0}^{B \times L D_{\mathrm{loc}}}$
    \For{$i = 0$ \textbf{to} $L-1$}
        \State $\mathrm{start}, \mathrm{end} \gets \mathrm{slices}[i]$
        \State $\mathrm{row}, \mathrm{col}, \mathrm{val} \gets \mathrm{rows}[\mathrm{start}:\mathrm{end}], \mathrm{cols}[\mathrm{start}:\mathrm{end}], \mathrm{vals}[\mathrm{start}:\mathrm{end}]$
        \State $V \gets$ \textproc{View}($W_{\mathrm{dec}}[i]$, $(F, (L-i) D_{\mathrm{loc}})$)
        \State $\mathrm{out} \gets \mathrm{recon}[:, i D_{\mathrm{loc}} :]$
            \Comment{view of layers $i$ to $L-1$}
        \If{\texttt{mode} $=$ \texttt{dense}}
            \State $\mathrm{out} \gets \mathrm{out} + {}$\textproc{Scatter}($\mathrm{row}$, $\mathrm{col}$, $\mathrm{val}$, $B$, $F$)\,$V$
                \Comment{materialise $A_i$}
        \ElsIf{\texttt{mode} $=$ \texttt{gather}}
            \State \textproc{IndexAdd}($\mathrm{out}$, $\mathrm{row}$, $V[\mathrm{col}] \odot \mathrm{val}$)
                \Comment{$(\mathrm{nnz}_i, (L-i) D_{\mathrm{loc}})$ temporary}
        \Else
            \State $\mathrm{out} \gets \mathrm{out} + {}$\textproc{EmbeddingBag}($\mathrm{col}$, $V$, \textproc{Offsets}($\mathrm{row}$), $\mathrm{val}$, \texttt{sum})
                \Comment{fused}
        \EndIf
    \EndFor
    \State \Return \textproc{View}($\mathrm{recon}$, $(B, L, D_{\mathrm{loc}})$)
\EndProcedure
\end{algorithmic}
\end{algorithm}

We implement three different numerically equivalent kernels to build the reconstruction tensor.

\begin{itemize}
    \item \texttt{dense} scatters the activations back to a dense buffer, and runs the original
    dense matmul.
    It is not sparsity aware but requires less communication column compared to sharding both the encoder and the decoder along \texttt{F}, a straightforward scheme for TP.
    \item \texttt{gather} gathers the selected rows of $W_{\mathrm{dec}}$ and then applies
    \texttt{index\_add}. It is sparsity aware but uses atomics.
    \item \texttt{embedding\_bag} fuses the gather, the scaling and the sum for each token. It
    materialises no $(\mathrm{nnz}_i, (L-i) D_{\mathrm{loc}})$ temporary and needs no atomics, and it is the
    kernel we recommend.
\end{itemize}

To avoid performance cliffs when sparsity collapses, each layer falls back to \texttt{dense} when
$\mathrm{nnz}_i > \rho B F$, where $\rho$ is a user-defined threshold that represents the maximum
tensor density to compute with the \texttt{gather} or the \texttt{embedding\_bag} kernel.

Compared to always sharding along the feature axis $F$, 
our \texttt{dense} kernel
does not reduce computation FLOPs. The FLOPs of one step are

\[
C_{\mathrm{enc}} = 4 B L F_{\mathrm{loc}} D, \qquad
C_{\mathrm{dec}}^{\mathrm{dense}} = \frac{6 B F D L (L+1)}{W},
\]
\[
C_{\mathrm{step}} = C_{\mathrm{enc}} + C_{\mathrm{dec}}^{\mathrm{dense}}
= \frac{2 B L F D}{W} \left(3L + 5\right).
\]

However, the pure-dense decoding scheme is memory bounded. Our \texttt{dense} kernel only requires
$1/W$ of the memory access of always sharding \texttt{F}. Meanwhile, our \texttt{dense} kernel requires about
$2BLD$ less communication volume. Together, the memory-access optimization and the communication
optimization significantly reduce the step time.

As for the \texttt{gather} and \texttt{embedding\_bag} kernels, the FLOPs of one step reduce
further, so these two kernels boost training performance,

\[
C_{\mathrm{dec}}^{\mathrm{sparse}}
= 6 \sum_{i} 2 \, \mathrm{nnz}_i \, (L-i) \, \frac{D}{W}
\approx 6 B K \frac{D}{W} (L+1),
\]
\[
C_{\mathrm{step}} = C_{\mathrm{enc}} + C_{\mathrm{dec}}^{\mathrm{sparse}}
= \frac{2 B D}{W} \left(2 L F + 3 K (L+1)\right).
\]

We compare the three kernels with the baseline, which shards along the feature axis $F$, on $128$ GPUs, each with 80GB VRAM, to show the advantage of sparse decode. As is shown in
\Cref{tab:sparse_decode_time}, when $k = 10$, $B=8192$, sparse decode with the \texttt{embedding\_bag} kernel
achieves about a $2.89\times$ speedup compared to the baseline. Specifically, when using the
\texttt{embedding\_bag} kernel, compute time reduces $65\%$ and communication time reduces $67\%$.

\begin{table}[htbp]
\centering
\small
\caption{Step time of the three sparse decode kernels and of the baseline, measured on $128$
Hopper GPUs at $k = 10$. Lower is better.}
\label{tab:sparse_decode_time}
\begin{tabular}{lccc}
\toprule
\textbf{Mode} & \textbf{Step time (s)} & \textbf{Compute and memory access (s)}
& \textbf{Communication (s)} \\
\midrule
baseline ($F$ sharded) & $1.025$ & $0.800$ & $0.224$ \\
\texttt{dense}                           & $0.552$ & $0.451$ & $0.101$ \\
\texttt{gather}                          & $0.436$ & $0.334$ & $0.102$ \\
\texttt{embedding\_bag}                  & $\mathbf{0.355}$ & $\mathbf{0.281}$ & $\mathbf{0.074}$ \\
\bottomrule
\end{tabular}
\end{table}

